$\texttt{COSMIC}$: Mutual Information for Task-Agnostic Summarization Evaluation

Assessing the quality of summarizers poses significant challenges. In response, we propose a novel task-oriented evaluation approach that assesses summarizers based on their capacity to produce summaries that are useful for downstream tasks, while preserving task outcomes. We theoretically establish a direct relationship between the resulting error probability of these tasks and the mutual information between source texts and generated summaries. We introduce $\texttt{COSMIC}$ as a practical implementation of this metric, demonstrating its strong correlation with human judgment-based metrics and its effectiveness in predicting downstream task performance. Comparative analyses against established metrics like $\texttt{BERTScore}$ and $\texttt{ROUGE}$ highlight the competitive performance of $\texttt{COSMIC}$.

==> tables/comprehensive_correlation_table_ct.tex <==
\begin{table}\centering
\caption{Established (reference-free) quality metrics Spearman correlation with performance on the downstream classification tasks. Where Sent. analysis stands for sentiment analysis, GPT det. for GPT detector, Policy for policy classification, Emotion for emotion classification and Emb. for paraphrase embedding.}
\label{tab:correlation_table_ct}
\resizebox{0.5\textwidth}{!}{\begin{tabular}{lrrrrr}
\toprule
 & Sent. analysis & GPT det. & Policy & Emotion & Emb. \\
Metric &  &  &  &  &  \\
\midrule
$I(\mathbf{S};\mathbf{T})$ & 0.65 & 0.73 & \bfseries 0.83 & 0.72 & \bfseries 0.79 \\
Attribution & 0.68 & 0.83 & 0.40 & 0.68 & 0.76 \\
Main ideas & 0.34 & 0.39 & 0.69 & 0.40 & 0.60 \\
\texttt{BARTScore} & 0.68 & 0.86 & 0.46 & 0.72 & 0.74 \\
\texttt{BERTScore} & \bfseries 0.70 & \bfseries 0.89 & 0.77 & \bfseries 0.75 & 0.69 \\
\texttt{ROUGE-L} & 0.54 & 0.65 & 0.71 & 0.58 & 0.29 \\
\bottomrule
\end{tabular}}
\end{table}


==> tables/correlation_table_full.tex <==
\begin{table}\centering
\caption{Correlation between MI and ROUGE, and Seahorse metrics and probability of success of the classifcation task, grouped by datasets for non-trivial decoding strategies. SH. stands for Seahorse metrics and CT. for classification tasks.}
\label{tab:correlation_table}
\resizebox{0.5\textwidth}{!}{\begin{tabular}{llrrrrrr}
\toprule
 & Metric & $I(S;T)$ & Attribution & Main ideas & \texttt{BARTScore} & \texttt{BERTScore} & \texttt{ROUGE-L} \\
\midrule
\multirow[c]{6}{*}{SH.} & Attribution & {\cellcolor[HTML]{26828E}} \color[HTML]{F1F1F1} 0.56 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 1.00 & {\cellcolor[HTML]{481B6D}} \color[HTML]{F1F1F1} 0.26 & {\cellcolor[HTML]{D2E21B}} \color[HTML]{000000} 0.95 & {\cellcolor[HTML]{3FBC73}} \color[HTML]{F1F1F1} 0.75 & {\cellcolor[HTML]{39568C}} \color[HTML]{F1F1F1} 0.42 \\
 & Comprehensible & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.11 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.07 & {\cellcolor[HTML]{375A8C}} \color[HTML]{F1F1F1} 0.42 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.10 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.02 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} -0.37 \\
 & Conciseness & {\cellcolor[HTML]{5EC962}} \color[HTML]{000000} 0.80 & {\cellcolor[HTML]{20A486}} \color[HTML]{F1F1F1} 0.67 & {\cellcolor[HTML]{65CB5E}} \color[HTML]{000000} 0.81 & {\cellcolor[HTML]{1FA188}} \color[HTML]{F1F1F1} 0.66 & {\cellcolor[HTML]{20A486}} \color[HTML]{F1F1F1} 0.67 & {\cellcolor[HTML]{481467}} \color[HTML]{F1F1F1} 0.24 \\
 & Grammar & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} -0.24 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} -0.35 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.16 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} -0.34 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} -0.30 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} -0.50 \\
 & Main ideas & {\cellcolor[HTML]{4AC16D}} \color[HTML]{000000} 0.77 & {\cellcolor[HTML]{481B6D}} \color[HTML]{F1F1F1} 0.26 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 1.00 & {\cellcolor[HTML]{471063}} \color[HTML]{F1F1F1} 0.23 & {\cellcolor[HTML]{33638D}} \color[HTML]{F1F1F1} 0.45 & {\cellcolor[HTML]{482475}} \color[HTML]{F1F1F1} 0.28 \\
 & Repetition & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} 0.01 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} -0.23 & {\cellcolor[HTML]{3D4D8A}} \color[HTML]{F1F1F1} 0.39 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} -0.23 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} -0.08 & {\cellcolor[HTML]{440154}} \color[HTML]{F1F1F1} -0.34 \\
\cline{1-8}
\multirow[c]{4}{*}{CT.} & Sentiment analysis & {\cellcolor[HTML]{1FA188}} \color[HTML]{F1F1F1} 0.65 & {\cellcolor[HTML]{22A785}} \color[HTML]{F1F1F1} 0.68 & {\cellcolor[HTML]{433E85}} \color[HTML]{F1F1F1} 0.34 & {\cellcolor[HTML]{22A785}} \color[HTML]{F1F1F1} 0.68 & {\cellcolor[HTML]{27AD81}} \color[HTML]{F1F1F1} 0.70 & {\cellcolor[HTML]{277F8E}} \color[HTML]{F1F1F1} 0.54 \\
 & GPT detector & {\cellcolor[HTML]{32B67A}} \color[HTML]{F1F1F1} 0.73 & {\cellcolor[HTML]{75D054}} \color[HTML]{000000} 0.83 & {\cellcolor[HTML]{3C4F8A}} \color[HTML]{F1F1F1} 0.39 & {\cellcolor[HTML]{8ED645}} \color[HTML]{000000} 0.86 & {\cellcolor[HTML]{A2DA37}} \color[HTML]{000000} 0.89 & {\cellcolor[HTML]{1F9E89}} \color[HTML]{F1F1F1} 0.65 \\
 & Policy classification & {\cellcolor[HTML]{70CF57}} \color[HTML]{000000} 0.83 & {\cellcolor[HTML]{3C508B}} \color[HTML]{F1F1F1} 0.40 & {\cellcolor[HTML]{25AC82}} \color[HTML]{F1F1F1} 0.69 & {\cellcolor[HTML]{31668E}} \color[HTML]{F1F1F1} 0.46 & {\cellcolor[HTML]{48C16E}} \color[HTML]{F1F1F1} 0.77 & {\cellcolor[HTML]{2DB27D}} \color[HTML]{F1F1F1} 0.71 \\
 & Emotion classification & {\cellcolor[HTML]{2FB47C}} \color[HTML]{F1F1F1} 0.72 & {\cellcolor[HTML]{23A983}} \color[HTML]{F1F1F1} 0.68 & {\cellcolor[HTML]{3B518B}} \color[HTML]{F1F1F1} 0.40 & {\cellcolor[HTML]{2EB37C}} \color[HTML]{F1F1F1} 0.72 & {\cellcolor[HTML]{40BD72}} \color[HTML]{F1F1F1} 0.75 & {\cellcolor[HTML]{238A8D}} \color[HTML]{F1F1F1} 0.58 \\
\cline{1-8}
Emb. & Emb. Paraphrase & {\cellcolor[HTML]{58C765}} \color[HTML]{000000} 0.79 & {\cellcolor[HTML]{42BE71}} \color[HTML]{F1F1F1} 0.76 & {\cellcolor[HTML]{218F8D}} \color[HTML]{F1F1F1} 0.60 & {\cellcolor[HTML]{37B878}} \color[HTML]{F1F1F1} 0.74 & {\cellcolor[HTML]{26AD81}} \color[HTML]{F1F1F1} 0.69 & {\cellcolor[HTML]{472A7A}} \color[HTML]{F1F1F1} 0.29 \\
\cline{1-8}
\multirow[c]{3}{*}{Common} & \texttt{ROUGE-L} & {\cellcolor[HTML]{26828E}} \color[HTML]{F1F1F1} 0.55 & {\cellcolor[HTML]{39568C}} \color[HTML]{F1F1F1} 0.42 & {\cellcolor[HTML]{482475}} \color[HTML]{F1F1F1} 0.28 & {\cellcolor[HTML]{34618D}} \color[HTML]{F1F1F1} 0.45 & {\cellcolor[HTML]{26AD81}} \color[HTML]{F1F1F1} 0.70 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 1.00 \\
 & \texttt{BERTScore} & {\cellcolor[HTML]{58C765}} \color[HTML]{000000} 0.79 & {\cellcolor[HTML]{3FBC73}} \color[HTML]{F1F1F1} 0.75 & {\cellcolor[HTML]{33638D}} \color[HTML]{F1F1F1} 0.45 & {\cellcolor[HTML]{6CCD5A}} \color[HTML]{000000} 0.82 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 1.00 & {\cellcolor[HTML]{26AD81}} \color[HTML]{F1F1F1} 0.70 \\
 & \texttt{BARTScore} & {\cellcolor[HTML]{23888E}} \color[HTML]{F1F1F1} 0.57 & {\cellcolor[HTML]{D2E21B}} \color[HTML]{000000} 0.95 & {\cellcolor[HTML]{471063}} \color[HTML]{F1F1F1} 0.23 & {\cellcolor[HTML]{FDE725}} \color[HTML]{000000} 1.00 & {\cellcolor[HTML]{6CCD5A}} \color[HTML]{000000} 0.82 & {\cellcolor[HTML]{34618D}} \color[HTML]{F1F1F1} 0.45 \\
\cline{1-8}
\bottomrule
\end{tabular}}
\end{table}


==> tables/model_summaries_table.tex <==
\begin{table}[H]\centering
\caption{Summary of the models we benchmarked with their name on the Huggingface hub, size and performance metrics.}
\label{tab:model_summaries}
\resizebox{\textwidth}{!}{\begin{tabular}{lllrrrrrrrr}
\toprule
 &  & Size & \texttt{ROUGE-L} & M. I. & Attr. & Rep. & Compr. & Conc. & Gram. & $I(T,S)$ \\
Model & Dataset &  &  &  &  &  &  &  &  &  \\
\midrule
\multirow[c]{3}{*}{Falconsai/medical\_summarization} & cnn\_dailymail & 60 M & 0.17 & 0.33 & 0.79 & 0.46 & 0.76 & 0.42 & 0.30 & 776.77 \\
 & multi\_news & 60 M & 0.10 & 0.22 & 0.73 & 0.47 & 0.72 & 0.36 & 0.36 & 760.28 \\
 & xsum & 60 M & 0.31 & 0.33 & 0.77 & 0.36 & 0.74 & 0.33 & 0.34 & 785.63 \\
\cline{1-11}
\multirow[c]{3}{*}{Falconsai/text\_summarization} & cnn\_dailymail & 60 M & 0.15 & 0.36 & 0.82 & 0.64 & 0.81 & 0.44 & 0.38 & 782.47 \\
 & multi\_news & 60 M & 0.10 & 0.23 & 0.80 & 0.60 & 0.75 & 0.38 & 0.38 & 764.71 \\
 & xsum & 60 M & 0.31 & 0.33 & 0.81 & 0.58 & 0.77 & 0.35 & 0.37 & 791.29 \\
\cline{1-11}
\multirow[c]{3}{*}{sshleifer/distilbart-xsum-12-1} & cnn\_dailymail & 221 M & 0.04 & 0.21 & 0.41 & 0.87 & 0.83 & 0.22 & 0.67 & 759.84 \\
 & multi\_news & 221 M & 0.03 & 0.17 & 0.42 & 0.82 & 0.77 & 0.23 & 0.68 & 752.15 \\
 & xsum & 221 M & 0.08 & 0.29 & 0.35 & 0.86 & 0.90 & 0.22 & 0.80 & 777.29 \\
\cline{1-11}
\multirow[c]{3}{*}{sshleifer/distilbart-cnn-6-6} & cnn\_dailymail & 229 M & 0.16 & 0.47 & 0.85 & 0.92 & 0.85 & 0.55 & 0.50 & 788.99 \\
 & multi\_news & 229 M & 0.10 & 0.34 & 0.86 & 0.90 & 0.84 & 0.52 & 0.57 & 771.95 \\
 & xsum & 229 M & 0.32 & 0.47 & 0.84 & 0.91 & 0.90 & 0.49 & 0.60 & 794.07 \\
\cline{1-11}
\multirow[c]{3}{*}{sshleifer/distilbart-xsum-6-6} & cnn\_dailymail & 229 M & 0.04 & 0.38 & 0.55 & 0.96 & 0.96 & 0.41 & 0.87 & 755.25 \\
 & multi\_news & 229 M & 0.03 & 0.33 & 0.57 & 0.95 & 0.94 & 0.44 & 0.88 & 743.97 \\
 & xsum & 229 M & 0.09 & 0.46 & 0.46 & 0.97 & 0.97 & 0.38 & 0.91 & 776.71 \\
\cline{1-11}
\multirow[c]{3}{*}{sshleifer/distilbart-cnn-12-3} & cnn\_dailymail & 255 M & 0.18 & 0.48 & 0.82 & 0.87 & 0.93 & 0.54 & 0.60 & 790.43 \\
 & multi\_news & 255 M & 0.10 & 0.36 & 0.82 & 0.86 & 0.92 & 0.53 & 0.66 & 772.01 \\
 & xsum & 255 M & 0.31 & 0.49 & 0.74 & 0.82 & 0.94 & 0.47 & 0.64 & 795.05 \\
\cline{1-11}
\multirow[c]{3}{*}{sshleifer/distilbart-cnn-12-6} & xsum & 305 M & 0.31 & 0.54 & 0.76 & 0.91 & 0.96 & 0.51 & 0.71 & 795.57 \\
 & multi\_news & 305 M & 0.11 & 0.39 & 0.84 & 0.89 & 0.93 & 0.57 & 0.69 & 774.02 \\
 & cnn\_dailymail & 305 M & 0.18 & 0.52 & 0.84 & 0.91 & 0.93 & 0.58 & 0.62 & 791.38 \\
\cline{1-11}
\multirow[c]{3}{*}{sshleifer/distill-pegasus-cnn-16-4} & cnn\_dailymail & 369 M & 0.13 & 0.48 & 0.83 & 0.81 & 0.92 & 0.54 & 0.64 & 787.41 \\
 & multi\_news & 369 M & 0.08 & 0.33 & 0.84 & 0.82 & 0.90 & 0.51 & 0.69 & 769.93 \\
 & xsum & 369 M & 0.23 & 0.47 & 0.81 & 0.84 & 0.94 & 0.49 & 0.70 & 792.68 \\
\cline{1-11}
\multirow[c]{3}{*}{sshleifer/distill-pegasus-xsum-16-4} & cnn\_dailymail & 369 M & 0.04 & 0.27 & 0.50 & 0.96 & 0.95 & 0.32 & 0.85 & 710.60 \\
 & xsum & 369 M & 0.08 & 0.44 & 0.45 & 0.97 & 0.97 & 0.36 & 0.91 & 779.85 \\
 & multi\_news & 369 M & 0.03 & 0.28 & 0.56 & 0.95 & 0.93 & 0.39 & 0.86 & 738.42 \\
\cline{1-11}
\multirow[c]{3}{*}{facebook/bart-large-cnn} & xsum & 406 M & 0.32 & 0.52 & 0.81 & 0.96 & 0.97 & 0.53 & 0.74 & 795.95 \\
 & multi\_news & 406 M & 0.10 & 0.37 & 0.86 & 0.95 & 0.94 & 0.58 & 0.73 & 772.67 \\
 & cnn\_dailymail & 406 M & 0.18 & 0.49 & 0.86 & 0.95 & 0.94 & 0.59 & 0.67 & 790.54 \\
\cline{1-11}
\multirow[c]{3}{*}{google/pegasus-multi\_news} & xsum & 570 M & 0.27 & 0.53 & 0.49 & 0.94 & 0.85 & 0.39 & 0.72 & 789.13 \\
 & multi\_news & 570 M & 0.13 & 0.40 & 0.70 & 0.91 & 0.79 & 0.46 & 0.63 & 771.39 \\
 & cnn\_dailymail & 570 M & 0.16 & 0.47 & 0.63 & 0.94 & 0.83 & 0.43 & 0.65 & 783.08 \\
\cline{1-11}
\multirow[c]{3}{*}{google/pegasus-large} & xsum & 570 M & 0.27 & 0.24 & 0.88 & 0.86 & 0.89 & 0.37 & 0.70 & 781.29 \\
 & multi\_news & 570 M & 0.12 & 0.17 & 0.82 & 0.72 & 0.77 & 0.39 & 0.47 & 768.02 \\
 & cnn\_dailymail & 570 M & 0.20 & 0.26 & 0.87 & 0.66 & 0.84 & 0.43 & 0.51 & 783.16 \\
\cline{1-11}
\multirow[c]{3}{*}{google/pegasus-arxiv} & xsum & 570 M & 0.14 & 0.11 & 0.32 & 0.25 & 0.43 & 0.13 & 0.28 & 735.51 \\
 & multi\_news & 570 M & 0.06 & 0.06 & 0.34 & 0.29 & 0.43 & 0.13 & 0.37 & 671.50 \\
 & cnn\_dailymail & 570 M & 0.10 & 0.08 & 0.35 & 0.26 & 0.45 & 0.12 & 0.30 & 718.14 \\
\cline{1-11}
\multirow[c]{3}{*}{mistralai/Mistral-7B-Instruct-v0.2} & multi\_news & 7241 M & 0.16 & 0.37 & 0.64 & 0.88 & 0.80 & 0.41 & 0.68 & 769.61 \\
 & cnn\_dailymail & 7241 M & 0.25 & 0.54 & 0.74 & 0.93 & 0.83 & 0.46 & 0.67 & 798.41 \\
 & xsum & 7241 M & 0.42 & 0.59 & 0.65 & 0.94 & 0.86 & 0.44 & 0.76 & 813.44 \\
\cline{1-11}
\bottomrule
\end{tabular}}
\end{table}

